Adaptive semiparametric Bayesian differential equations via sequential Monte Carlo

Nonlinear differential equations (DEs) are used in a wide range of scientific problems to model complex dynamic systems. The differential equations often contain unknown parameters that are of scientific interest, which have to be estimated from noisy measurements of the dynamic system. Generally, there is no closed-form solution for nonlinear DEs, and the likelihood surface for the parameter of interest is multi-modal and very sensitive to different parameter values. We propose a Bayesian framework for nonlinear DE systems. A flexible nonparametric function is used to represent the dynamic process such that expensive numerical solvers can be avoided. A sequential Monte Carlo algorithm in the annealing framework is proposed to conduct Bayesian inference for parameters in DEs. In our numerical experiments, we use examples of ordinary differential equations and delay differential equations to demonstrate the effectiveness of the proposed algorithm. We developed an R package that is available at \url{https://github.com/shijiaw/smcDE}.

==> macros-topic.tex <==
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{epsfig}

\DeclareMathOperator{\prop}{prop}

\def\half{\frac{1}{2}}

\def\randomgraph{{\cal G}_{n,\frac{1}{2}}}
\def\scrp{{\mathscr P}}
\def\scrc{{\mathscr C}}
\def\scre{{\mathscr E}}

\newcounter{xxx}
\setcounter{xxx}{0}
\newcommand\XXX[1]{{\bf \em \addtocounter{xxx}{1} (\thexxx) [[#1]]}}

% \DeclareMathOperator{\deg}{deg} 



\def\Q{{\mathbb Q}}        % rationals
\def\F{{\mathbb F}}        % rationals
\def\Z{{\mathbb Z}}        % integers
\def\N{{\mathbb N}}        % naturals
\def\R{{\mathbb R}}        % reals
\def\C{{\mathbb C}} 	   % complex
\def\Rn{{\R^{n}}}          % product of n copies of reals
\def\Cf{{\mathbf C}}	   % continuous functions on (.)

\def\P{{\mathbb P}}        % probability
\def\E{{\mathbb E}}        % expectation 
\def\1{{\mathbf 1}}        % indicator
\def\var{{\mathop{\mathbf Var}}}    % variance

\def\done{\hfill\rule{2mm}{2mm}}

\def\borel{{\cal B}}    % borel sigmal field
\def\G{{\cal G}}        % some sigma field
\def\F{{\cal F}}        % some sigma field
\def\H{{\cal H}}        % some sigma field

\def\L{{\mathbf L}}     % L, as in L^2

\def\iid{\stackrel{\scriptscriptstyle iid}{\sim}}   

\def\ascv{\stackrel{\scriptscriptstyle a.s.}{\longrightarrow}}     % almost sure convergnece
\def\pcv{\stackrel{\scriptscriptstyle \P}{\longrightarrow}}        % convergence in P
\def\ltcv{\stackrel{\scriptscriptstyle\L^2}{\longrightarrow}}      % L2 convergnece
\def\lpcv{\stackrel{\scriptscriptstyle\L^p}{\longrightarrow}}      % Lp convergnece
\def\dcv{\stackrel{\scriptscriptstyle d}{\longrightarrow}}         % convergence in d
\def\deq{\stackrel{\scriptscriptstyle d}{=}}			   % equal in d
\def\toinf{\to \infty}

\def\ci{\perp\!\!\!\perp}  % conditional independence

% the header/lecture structure...borrowed from alistair sinclair's cs270 format
% \newcommand{\topic}[3]{
%    \pagestyle{myheadings}
%    \thispagestyle{plain}
%    \newpage
%    \setcounter{page}{1}
%    \noindent
%    \begin{center}
%    \framebox{
%       \vbox{\vspace{2mm}
%     \hbox to 6.28in { {\bf STAT 205~Probability Theory
%                         \hfill Fall 2006} }
%        \vspace{4mm}
%        \hbox to 6.28in { {\Large \hfill Topic: #1 \hfill} }
%        \vspace{2mm}
%        \hbox to 6.28in { {\it Lecturer:} Jim Pitman, {\it Scribe:} #2, {\it Editor:} #3 \hfill }
%       \vspace{2mm}}
%    }
%    \end{center}
%    \markboth{Topic: #1}{Topic: #1}
%    \vspace*{4mm}
% }
       %\hbox to 5.90in { \hfill {\it Scribe: #3} }


%\newenvironment{proof}{{\bf Proof:}}{\hfill\rule{2mm}{2mm}}
\newenvironment{proofsketch}{{\bf Proof Sketch:}}{\hfill\rule{2mm}{2mm}}
\newcommand{\fig}[3]{
      \vspace{#2}
      \begin{center}
      Figure #1:~#3
      \end{center}
}


% %some things we'll never understand....alas
% \setlength{\oddsidemargin}{0.25 in}
% \setlength{\evensidemargin}{-0.25 in}
% \setlength{\topmargin}{-0.6 in}
% \setlength{\textwidth}{6.0 in}
% \setlength{\textheight}{8.5 in}
% \setlength{\headsep}{0.75 in}
% \setlength{\parindent}{0 in}
% \setlength{\parskip}{0.1 in}
% \advance\topmargin by 0.5in



\newcommand\bracearray[1]{\left\{ \begin{array}{l} #1 \end{array} \right.}
\newcommand\bracearraypair[2]{\bracearray{#1 \\ #2}}
\newcommand\bracearraytriple[3]{\bracearray{#1 \\ #2 \\ #3}}
\newcommand\bracearrayquad[4]{\bracearray{#1 \\ #2 \\ #3 \\ #4}}
\newcommand\dotprod[2]{\langle #1, #2\rangle}

\newcommand\partialderiv{\frac{\partial}{\partial \theta_i}}
\newcommand\bracearraycond[1]{\left\{ \begin{array}{ll} #1 \end{array} \right.}


\newcommand\poset{\mathcal S}
\newcommand\target{\mathcal X}
\newcommand\sigmaalg{{\mathcal F}}
\newcommand\observations{\mathcal Y}




\newcommand\X{{\cal X}}
\newcommand\ps{ E}  % partial states
\newcommand\sps{{\cal E}}  

\newcommand{\ud}{\,\mathrm{d}}
%\newcommand{\path}{{\mathbf s}}

%\def\law{\rightarrow_d}
\newcommand{\bigone}{{\rm 1\hspace{-3 pt}l}}

\newcommand{\ybold}    {\mbox{\bf y}}

\newcommand{\chatbold} {\widehat{\mbox{\bf c}}}
\newcommand{\dhatbold} {\widehat{\mbox{\bf d}}}
\newcommand{\xhatbold} {\widehat{\mbox{\bf x}}}
\newcommand{\yhatbold} {\widehat{\mbox{\bf y}}}
\newcommand{\Ahatbold} {\widehat{\mbox{\bf A}}}
\newcommand{\Bhatbold} {\widehat{\mbox{\bf B}}}
\newcommand{\Qhatbold} {\widehat{\mbox{\bf Q}}}
\newcommand{\Rhatbold} {\widehat{\mbox{\bf R}}}
\newcommand{\Yhatbold} {\widehat{\mbox{\bf Y}}}





\newcommand{\bboldhat}    {\widehat{\mbox{\bf b}}}
\newcommand{\cboldhat}    {\widehat{\mbox{\bf c}}}
\newcommand{\xboldhat}    {\widehat{\mbox{\bf x}}}
\newcommand{\yboldhat}    {\widehat{\mbox{\bf y}}}
\newcommand{\Rboldhat}    {\widehat{\mbox{\bf R}}}

\newcommand{\Ibold}     {\mbox{\boldmath${I}$}}
\newcommand{\abold}     {\mbox{\boldmath${a}$}}
\newcommand{\sbold}     {\mbox{\boldmath${s}$}}
\newcommand{\varrhobold}     {\mbox{\boldmath${\varrho}$}}
\newcommand{\taubold}     {\mbox{\boldmath${\tau}$}}
\newcommand{\Pbold}     {\mbox{\boldmath${\mathcal P}$}}
\newcommand{\pibold}     {\mbox{\boldmath${\pi}$}}
\newcommand{\varphibold}   {\mbox{\boldmath${\varphi}$}}
\newcommand{\alphabold}   {\mbox{\boldmath${\alpha}$}}
\newcommand{\betabold}    {\mbox{\boldmath${\beta}$}}
\newcommand{\epsilonbold} {\mbox{\boldmath${\epsilon}$}}
\newcommand{\etabold}     {\mbox{\boldmath${\eta}$}}
\newcommand{\gammabold}   {\mbox{\boldmath${\gamma}$}}
\newcommand{\lambdabold}  {\mbox{\boldmath${\lambda}$}}
\newcommand{\rhobold}  {\mbox{\boldmath${\rho}$}}
\newcommand{\mubold}      {\mbox{\boldmath${\mu}$}}
\newcommand{\phibold}     {\mbox{\boldmath${\phi}$}}
\newcommand{\Phibold}     {\mbox{\boldmath${\Phi}$}}
\newcommand{\psibold}     {\mbox{\boldmath${\psi}$}}
\newcommand{\Psibold}     {\mbox{\boldmath${\Psi}$}}
\newcommand{\thetabold}   {\mbox{\boldmath${\theta}$}}
\newcommand{\Thetabold}   {\mbox{\boldmath${\Theta}$}}
\newcommand{\Sigmabold}   {\mbox{\boldmath${\Sigma}$}}
\newcommand{\Sigb}        {\mbox{\boldmath${\Sigma}$}}
\newcommand{\xibold}      {\mbox{\boldmath${\xi}$}}
\newcommand{\zetabold}    {\mbox{\boldmath${\zeta}$}}
\newcommand{\trace}    {\mbox{trace}}
\newcommand{\aboldhat} {\widehat{\mbox{\boldmath${a}$}}}
% \newcommand{\bboldhat} {\widehat{\mbox{\boldmath${b}$}}}
\newcommand{\lambdaboldhat} {\widehat{\mbox{\boldmath${\lambda}$}}}
\newcommand{\betaboldhat} {\widehat{\mbox{\boldmath${\beta}$}}}
\newcommand{\thetaboldhat} {\widehat{\mbox{\boldmath${\theta}$}}}
\newcommand{\Sigmaboldhat} {\widehat{\mbox{\boldmath${\Sigma}$}}}
\newcommand{\muboldhat} {\widehat{\mbox{\boldmath${\mu}$}}}

\newcommand{\INDSTATE}[1][1]{\STATE\hspace{#1\algorithmicindent}}


